LLM as OS, Agents as Apps: Envisioning AIOS, Agents and the AIOS-Agent Ecosystem

This paper envisions a revolutionary AIOS-Agent ecosystem, where Large Language Model (LLM) serves as the (Artificial) Intelligent Operating System (IOS, or AIOS)--an operating system "with soul". Upon this foundation, a diverse range of LLM-based AI Agent Applications (Agents, or AAPs) are developed, enriching the AIOS-Agent ecosystem and signaling a paradigm shift from the traditional OS-APP ecosystem. We envision that LLM's impact will not be limited to the AI application level, instead, it will in turn revolutionize the design and implementation of computer system, architecture, software, and programming language, featured by several main concepts: LLM as OS (system-level), Agents as Applications (application-level), Natural Language as Programming Interface (user-level), and Tools as Devices/Libraries (hardware/middleware-level). We begin by introducing the architecture of traditional OS. Then we formalize a conceptual framework for AIOS through "LLM as OS (LLMOS)", drawing analogies between AIOS and traditional OS: LLM is likened to OS kernel, context window to memory, external storage to file system, hardware tools to peripheral devices, software tools to programming libraries, and user prompts to user commands. Subsequently, we introduce the new AIOS-Agent Ecosystem, where users can easily program Agent Applications (AAPs) using natural language, democratizing the development of software, which is different from the traditional OS-APP ecosystem. Following this, we explore the diverse scope of Agent Applications. We delve into both single-agent and multi-agent systems, as well as human-agent interaction. Lastly, drawing on the insights from traditional OS-APP ecosystem, we propose a roadmap for the evolution of the AIOS-Agent ecosystem. This roadmap is designed to guide the future research and development, suggesting systematic progresses of AIOS and its Agent applications.

==> sections/old_Background.tex <==
\section{Background}
What exactly are agents? What properties should they have, and how are we to formally represent and reason about these properties?

\subsection{What is an agent?}

An agent refers to an artificial entity capable of perceiving its surroundings using sensors, making decisions, and then taking actions in response using actuators. 

% As AI advanced, the term ``agent'' found its place in AI research to depict entities showcasing intelligent behavior and possessing qualities like autonomy, reactivity, pro-activeness, and social ability.

% \subsection{ What properties should they have?}
Researchers have introduced several properties to help describe and define agents in the field of AI \cite{shehory2014brief}. Here, we will delve into some key properties, elucidate their relevance to LLMs, and thereby expound on why LLMs are highly suited to serve as the main part of brains of AI agents.

\begin{itemize}
    \item \textbf{Autonomy}: 
    means that an agent operates without direct intervention from humans or others and possesses a degree of control over its actions and internal states [4; 113]. This implies that an agent should not only possess the capability to follow explicit human instructions for task completion but also exhibit the capacity to initiate and execute actions independently. 

    \item \textbf{Intelligence}: \citet{laird2020intelligence} equate intelligence with rationality, where an agent uses its available knowledge to select the best action(s) to achieve its goal(s) within an environment. This perspective posits that intelligence is the extent to which an agent's behavior, or actions, is optimal relative to its available knowledge and the tasks it must perform. A task is defined as a set of goals situated within an environment. While it is common in the field of AI to measure intelligence in the context of a single task, it is also pertinent to evaluate intelligence across a series or collection of tasks, where the knowledge acquired during earlier tasks can impact the performance of an agent in subsequent tasks.

    \item \textbf{Interactive}: \citet{franklin1996agent} highlight a fundamental distinction between autonomous agents and computer programs, which is, while programs, even those based on machine learning models, are crafted to address individual inputs or queries, autonomous agents, on the other hand, must continuously interact with their environment or with other agents over an extended duration.


    \item \textbf{Sociality.} In many cases, an agent is situated in a multi-agent environment. To meet its goals, the agent may need to interact with other agents and coordinate, collaborate, or compete with them. For instance, an agent may need to form a team to perform a rescue task in a disaster recovery mission. To facilitate such capabilities, the architecture of the agent should include sociality-supporting constructs. At the infrastructural level, communication is required.


    % \item \textbf{Mobility.} Some agents and multi-agent systems exhibit mobility. That is, agents may be able to change their logical or physical location. One way of mobility manifestation is for the agent to move from its current execution environment (the host on which it runs) to another execution environment. Another incarnation of mobility is found in cases where agents reside on mobile devices such as smartphones. In such cases, even if the agent never leaves its host, the hosting device itself may roam, thus changing location and environmental conditions. As a result, the agent that executes on the device roams and changes its environmental conditions as well. Both types of mobility require that agents be designed for mobility and be equipped with the proper software artifacts to manage it.
\end{itemize}







% \subsection{Architecture}
% CoALA \cite{sumers2023cognitive} 

% \citet{weng2023prompt}
\subsection{How LLMs satisfy the properties?}
LLMs showcase remarkable autonomy, intelligence, and interactivity, demonstrating capabilities that extend far beyond mere text generation. They have the capacity to autonomously generate human-like text, conduct engaging conversations, and accomplish various tasks without the need for meticulous step-by-step instructions, illustrating a profound form of autonomous operation \cite{Significant_Gravitas_Auto-GPT,openagi}. Beyond this, LLMs exhibit a form of creative autonomy, where they can invent novel ideas, narratives, or solutions that are not explicitly programmed into them, reflecting an advanced level of creative intelligence \cite{yuan2022wordcraft,franceschelli2023creativity}. This ability to generate new, unprecedented content implies a level of self-directed exploration and decision-making, highlighting their advanced cognitive capabilities.
Auto-GPT is a prime example of how LLMs serve as autonomous agents with extensive potential, by autonomously formulating and executing plans to accomplish given tasks using available tools, thus achieving predetermined goals \cite{Significant_Gravitas_Auto-GPT}. This demonstrates not only their autonomous capabilities but also their intelligence and interactive abilities, as they can comprehend tasks, strategize, and implement solutions while dynamically interacting with the environment or user inputs.

Moreover, LLMs can intelligently modify their outputs in response to environmental inputs, showcasing adaptive autonomy that is reflected in their ability to dynamically interact with their surroundings \cite{wang2023interactive,liu2023training,liu2023languages}. This adaptiveness is a marker of their intelligent responsiveness to the contextual inputs they receive, allowing for more nuanced and relevant interactions.







\subsection{Benefits}
\subsubsection{LLMs for Agents}
Emergent abilities of LLMs. LLMs exhibit remarkable abilities to solve new tasks from just a few examples or textual instructions, especially at scale.




Language agents have the potential to be more explainable to humans, since we expect natural language explanations to be more intuitively understood by humans than explanations by a robot acting in the physical world. Explainability is important since we want to be able to trust that our agents are beneficial before deploying them.

\subsubsection{Agents for LLMs}

==> sections/old_Discussion.tex <==
% \section{Discussion}



% \section{Discussion} \label{sec:discussion}




% \subsection{Human-Agent Ecosystem}


% \subsection{Agent Governance}



% \subsection{Limitation of Current Evaluation Methods}






==> sections/old_Human_Agents.tex <==
\section{Human-Agent Interaction}
Existing agent frameworks generally define and control the agents’ behavior only using a system prompt and then let the agent plan and act on its own.

AgentVerse \cite{chen2023agentverse} simulates the problem-solving procedures of human groups, and allows for dynamic adjustment of group members based on current problem-solving progress. Specifically, it splits the group problem-solving process into four pivotal stages, which are (1) Expert Recruitment; (2) Collaborative Decision-Making; (3) Action Execution; (4) Evaluation.

AutoGen \cite{wu2023autogen} is an open-source framework that allows developers to build LLM applications via multiple agents that can converse with each other to accomplish tasks. AutoGen agents are customizable, conversable, and can operate in various modes that employ combinations of LLMs, human inputs, and tools.

AutoAgents \cite{chen2023autoagents} is a framework that adaptively generates and coordinates multiple specialized agents to build an AI team according to different tasks. Specifically, it couples the relationship between tasks and roles by dynamically generating multiple required agents based on task content and planning solutions for the current task based on the generated expert agents.


AGENTS \cite{zhou2023agents} provides a novel paradigm to build controllable agents via a symbolic plan, also referred to as standard operating procedures (SOPs), which can be generated by an LLM and edited by the user when customizing and tuning the agent.


==> sections/old_Multi_Agents.tex <==
\section{Multi-Agent Systems}

% \subsection{Learning Strategies}
How can communication emerge? A necessary prerequisite is a task that requires coordination between multiple agents to solve, and some communication protocol for the agents to exchange messages through.

Multi-agent systems offer a way to study how communication could emerge in communities of agents needing to solve specific problems. 

\subsection{Applications}

\subsubsection{Collaborative Interaction} Given the expanding tasks that could benefit from LLMs and the growing task complexity, an intuitive approach to scale up the power of agents is to use multiple agents that cooperate. Collaborative multi-agent systems are the most widely deployed pattern in practical usage. Within such systems, individual agent assesses the needs and capabilities of other agents and actively seeks collaborative actions and information sharing with them \cite{li2023camel}.



\textbf{Non-player Characters (NPCs).} 

Generative Agents \cite{park2023generative} are believable simulacra of human behavior for interactive applications. In this work, we demonstrate generative agents by populating a sandbox environment, reminiscent of The Sims, with twenty-five agents. Users can observe and intervene as agents plan their days, share news, form relationships, and coordinate group activities.

Humanoid Agents \cite{wang2023humanoid} is a system that guides Generative Agents to behave more like humans by introducing three elements of System 1 processing: Basic needs (e.g. hunger, health and energy), Emotion and Closeness in Relationships.

\textbf{Software Development.}


MetaGPT\cite{hong2023metagpt} is a specialized LLM application based on a multi-agent conversation framework for automatic software development by assigning different roles to GPTs to collaboratively develop software applications.

BOLAA \cite{liu2023bolaa} has a controller module on top of multiple collaborated agents, for enabling the selection and communication between multiple labor agents.

% GameGPT \cite{chen2023gamegpt}

CHATDEV \cite{qian2023communicative} presents a novel software development framework that harnesses agents to enhance
collaboration among the various roles involved in the software development process.

\textbf{Conversation}

Negotiation is semi-collaborative setting. For example, \cite{fu2023improving} studies whether large language models can autonomously improve their negotiation skills by playing a bargaining game against each other and incorporating natural language feedback from an AI critic.


\subsubsection{Adversarial Interaction}
Traditionally, collaborative methods have been extensively explored in multi-agent systems. However, researchers are increasingly recognizing that introducing concepts from game theory into systems can lead to more robust and efficient behaviors.


\textbf{Debate}

In reasoning tasks, \citet{du2023improving} introduce the concept of debate, endowing agents with responses from fellow peers. When these responses diverge from an agent’s own judgments, a “mental” argumentation occurs, leading to refined solutions. ChatEval \cite{chan2023chateval} establishes a role-playing-based multi-agent referee team. Through self-initiated debates, agents evaluate the quality of text generated by LLMs, reaching a level of excellence comparable to human evaluators.

Corex \cite{sun2023corex} is constituted by diverse collaboration paradigms including Debate, Review, and Retrieve modes, which collectively work towards enhancing the factuality, faithfulness, and reliability of the reasoning process. These paradigms foster task-agnostic approaches that enable LLMs to ``think outside the box'', thereby overcoming hallucinations and providing better solutions.

MAD (Multi-Agent Debate) \cite{liang2023encouraging} is a framework wherein several agents engage in a ``tit-for-tat'' exchange of arguments under the oversight of a judge who steers the discussion towards a conclusive solution.


\subsection{Evaluation}


\subsection{Toolkit and Frameworks}
BabyAGI \cite{babyagi2023} is an example implementation of an AI-powered task management system in a Python script. In this implemented system, multiple LLM-based agents are used. For example, there is an agent for creating new tasks based on the objective and the result of the previous task, an agent for prioritizing the task list, and an agent for completing tasks/sub-tasks.

AgentVerse \cite{chen2023agentverse} is a versatile framework that helps researchers quickly create customized multiple LLM-based agent simulations.  

Camel \cite{li2023camel} is a communicative agent framework. It demonstrates how role playing can be used to let chat agents communicate with each other for task completion. It also records agent conversations for behavior analysis and capability understanding. An Inception-prompting technique is used to achieve autonomous cooperation between agents.

% Langroid \footnote{https://github.com/langroid/langroid}


\subsection{Open Problems and Future Directions}
\subsubsection{Memory Explosion}


\subsubsection{Communication Between Agents}
Natural conversations involve a rapid exchange of utterances where speakers coordinate on-the-fly to avoid talking over each other. This turn-taking phenomenon is ubiquitous across cultures \cite{stivers2009universals} and is even found in some forms of animal communication \cite{pika2018taking,demartsev2018vocal}. The ability to engage in spontaneous turn-taking develops early in humans, even before linguistic competence \cite{nguyen2022systematic} and allows us to hold fluent conversations with very little downtime between utterances \cite{heldner2010pauses}. In contrast, fluid turn-taking is difficult to replicate in artificial dialogue systems. Modern conversational agents often rely on explicit cues, for instance pressing ``enter'' in text-based chatbots, the use of specific wake-words \cite{gao2020towards}, or long silences of pre-determined length\cite{skantze2021turn}.  Given these observations, an interesting question to ask is what task structures aid the emergence of communication and how different communication protocols affect task success.


\subsubsection{Society of Mind}

==> sections/old_Single_Agent.tex <==
\section{Single Agents}

\begin{table}
\centering
\caption{Comparison of Language Agent Frameworks}
\begin{tabularx}{\textwidth}{l|cccc}
\toprule
Framework & Tool Usage & Long-short Term Memory & Multi-Agent & Human-Agent Interaction \\
\midrule
Transformers Agents & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
LangChain & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
Auto-GPT & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
Gentopia & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
XLang & $\checkmark$ & $\times$ & $\times$ & $\times$ \\
Meta-GPT & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
Camel & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
AgentVerse & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ \\
AGENTS & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
\bottomrule
\end{tabularx}
\end{table}

\subsection{Applications}
%物理 网络 虚拟世界 
%Physical Space, Cyber Space (internet), Simulation Space (Minecraft, simulated driving environment, simulated robotics, etc.)
%学科

% \subsection{Environment}

We categorize three kinds of external environments:

% \textbf{Physical environments.} 

% \textbf{Cyber environments.} 

% \textbf{Simulated Environment.} 

\subsubsection{Physical Environment}The focus is on enhancing autonomous agents’ abilities for planning, reasoning, and collaboration in embodied environments.

Physical embodiment is the oldest instantiation envisioned for AI agents \cite{nilsson1984shakey}. It involves processing perceptual inputs (visual, audio, tactile) into textual observations (e.g., via pre-trained captioning models), and affecting the physical environments via robotic planners that take language-based commands. Recent advances in LLMs have led to numerous robotic projects \cite{ahn2022can,liang2023code,singh2023progprompt,di2023towards,ren2023robots} that leverage LLMs as a “brain” for robots to generate actions or plans in the physical world. For perceptual input, vision-language models are typically used to convert images to text \cite{alayrac2022flamingo,sumers2023distilling} providing additional context for the LLM \cite{driess2023palm,huang2023instruct2act,brohan2022rt,zitkovich2023rt}.

\cite{li2023multimodal}

\textbf{Scientific Research.}

Agents have the capacity to function autonomously, undertaking experiments independently, while also serving as invaluable resources for scientists engaged in research projects \cite{boiko2023emergent, bran2023chemcrow}. For instance, the agent system depicted in \cite{boiko2023emergent} integrates AI modules, software tools, reasoning capabilities, and lab hardware into an end-to-end platform that automates key aspects of scientific experimentation. It gathers information online, analyzes prompts to design experiments, runs calculations and protocols using Python and lab APIs, controls robotic equipment, adapts to errors, refuses unethical requests, and leverages analytical tools - combining diverse capabilities for autonomous experimentation from information search to result analysis. Moreover, ChemCrow \cite{bran2023chemcrow} encompasses a suite of 17 meticulously devised tools, tailored explicitly to assist researchers conducting chemical investigations. Upon receipt of the input objectives, ChemCrow proffers insightful suggestions for experimental methodologies, meticulously underscoring potential safety hazards linked to the suggested experiments.

\cite{huang2023benchmarking} propose MLAgentBench, a suite of ML tasks for benchmarking AI research agents

\textbf{Robotics.}

ChatGPT for Robotics \cite{vemprala2023chatgpt} employs ChatGPT for a wide array of robotics tasks through strategic prompt engineering, showing its ability to comprehend and respond to natural language instructions in the context of robotics applications.

SayCan \cite{ahn2022can} is instrumental in extracting and utilizing the knowledge encapsulated within Large Language Models (LLMs). It comprises two integral components: the ``Say'' part of the LLM, responsible for task-grounding by identifying pertinent actions for a high-level objective, and the ``Can'' part, which encompasses learned affordance functions that offer a world-grounding, thereby determining the feasible actions for the plan's execution. The system employs reinforcement learning (RL) to ascertain language-conditioned value functions, thereby delineating the possible affordances in the world. This method ensures not only the relevance of the actions chosen for the specified task but also their feasibility in the real-world scenario, consequently contributing to the development of more intelligent and adaptable systems.
% \cite{reed2022generalist}

VOYAGER \cite{wang2023voyager} presents lifelong learning with prompting mechanisms, skill library, and self-verification, which are based on LLM. These three modules aim to enhance the development of more complex behaviors of agents. 

EUREKA (Evolution-driven Universal REward Kit for Agent) \cite{ma2023eureka}, a novel reward design algorithm powered by coding LLMs 
\cite{wang2023prompt}

 Robotic Learning Datasets and RT-X Models \cite{embodimentcollaboration2023open}

% Habitat 3.0 \cite{puig2023habitat3}
 
\textbf{Autonomous Driving.}

% \cite{DriveLM_Contributors_Drive_on_Language_2023}
\citet{fu2023drive} propose an agent-based autonomous driving system, which widely adopts a four-module framework: Environment, Agent, Memory, and Expert. The Environment sets the interaction stage, the Agent perceives the environment and decides, the Memory accumulates experience for action, and the Expert provides training advice and inconsistency feedback. In a universal driving framework, these modules can be represented by the real world or simulator, human drivers or algorithms, and simulator or instructor feedback, respectively.

\subsubsection{Cyber Environment}
This mainly includes APIs \cite{schick2023toolformer,yao2023impact,parisi2022talm,tang2023toolalpaca}, and websites \cite{} as well as general code execution \cite{}. Such digital grounding is cheaper and faster than physical or human interaction. It is thus a convenient testbed for language agents and has been studied with increasing intensity in recent years. In particular, for NLP tasks that require augmentation of external knowledge or computation, stateless digital APIs (e.g., search, calculator, translator) are often packaged as ``tools'' \cite{}, which can be viewed as special ``single-use'' digital environments.

MusicAgent \cite{yu2023musicagent} integrates numerous music-related tools and an autonomous workflow to address user requirements.

Auto-UI \cite{zhan2023you} is a multi-modal solution that directly interacts with the interface, bypassing the need for environment parsing or reliance on application-dependent APIs.


\textbf{Recommendation.} Recent literature demonstrates the efficacy of employing agents in recommender systems \cite{wang2023recagent, wang2023recmind, feng2023large}. For instance, the LLMCRS (Large Language Model Enchanced Conversational Recommendation System) \cite{feng2023large} is a specialized conversational recommendation agent. This system employs Large Language Models (LLMs) to manage sub-tasks during the conversational recommendation process efficiently. Additionally, LLMCRS fosters collaboration between LLMs and various expert models, each specializing in different sub-tasks, thereby enhancing the performance of individual sub-tasks collectively. Lastly, the system leverages the LLM as a language interface to generate refined and improved responses to users. This holistic approach optimizes sub-task management and performance, leading to a significant improvement in the quality of responses in conversational recommendation systems.






\textbf{Coding.} ToolCoder, developed by \citet{zhang2023toolcoder}, combines API search tools with existing models to aid in code generation and API selection. This approach consists of a two-step process: firstly, an automated data annotation technique, powered by ChatGPT, is employed to incorporate tool usage data into the source code. Subsequently, the code generation model undergoes a fine-tuning phase. Remarkably, during the inference stage, the API search tool is seamlessly incorporated into the generation workflow, thereby enabling the model to autonomously leverage the tool in providing suggestions for API selection. This integration not only optimizes the code generation process but also enhances the model's ability to make informed decisions when selecting APIs.

Lemur-series models \cite{xu2023lemur} are meticulously pre-trained and instruction fine-tuned to demonstrate balanced language and coding capabilities.

\textbf{Web.} WorkGPT\footnote{https://github.com/team-openpm/workgpt}, and SuperAGI\footnote{https://github.com/TransformerOptimus/SuperAGI}, to name a few. 
WorkGPT [32] is an agent framework similar to AutoGPT and LangChain. By providing it with an instruction and a set of APIs, it engages in back-and-forth conversations with AI until the instruction is completed. AGiXT [40] is a dynamic AI automation platform designed to orchestrate efficient AI command management and task execution across many providers. 

Auto-GPT \cite{Significant_Gravitas_Auto-GPT} stands out as an automated agent, which is designed to set multiple objectives, break them down into relevant tasks, and iterate on these tasks until the objectives are achieved.

BMTools \cite{qin2023tool} is an open-source repository that extends LLMs with tools and provides a platform for community-driven tool building and sharing. It supports various types of tools, enables simultaneous task execution using multiple tools, and offers a simple interface for loading plugins via URLs, fostering easy development and contribution to the BMTools ecosystem.


\subsubsection{Simulated Environment}
This includes interacting with games \cite{hausknecht2020interactive,cote2019textworld,shridhar2020alfworld,wang2022scienceworld，liu2022mind}

\textbf{Minecraft Game.} MINECLIP agents, introduced by \citet{fan2022minedojo}, is a novel agent learning algorithm that leverages large pre-trained video-language models as a learned reward function. Specifically, the authors first proposed MINEDOJO, a new framework built on the popular Minecraft game that features a simulation suite with thousands of diverse open-ended tasks and an internet-scale knowledge base with Minecraft videos, tutorials, wiki pages, and forum discussions. 

\subsubsection{Hybrid Environment}
A number of open source projects based on LLM development have conducted preliminary explorations of AGI, they are dedicated to the autonomous universal AI agent framework, enabling developers to build, manage, and run useful autonomous agents quickly and reliably. 



% \cite{patil2023gorilla}





\subsection{Dataset and Benchmarks}
With the rising interest and attention from researchers and practitioners in this area of study, there has been a notable increase in the availability of datasets and benchmarks, indicating its growing significance.

WebShop \cite{yao2022webshop} is a recently proposed online shopping website environment with 1.18M real-world products and 12k human instructions, containing a high variety of structured and unstructured texts (e.g. product titles, descriptions, and options crawled from Amazon), and requires an agent to purchase a product based on a user instruction.


FEVER \cite{thorne2018fever}, a fact verification benchmark where each claim is annotated SUPPORTS, REFUTES, or NOT ENOUGH INFO, based on if there exists a Wikipedia passage to verify the claim. 

ALFWorld \cite{shridhar2020alfworld} is a synthetic text-based game designed to align with the embodied ALFRED benchmark \cite{shridhar2020alfred}. It includes 6 types of tasks in which an agent needs to achieve a high-level goal (e.g. examine paper under desklamp) by navigating and interacting with a simulated household via text actions (e.g. go to coffee table 1, take paper 2, use desklamp 1). A task instance can have more than 50 locations and take an expert policy more than 50 steps to solve, thus challenging an agent to plan and track sub-goals, as well as explore systematically (e.g. check all desks one by one for desklamp). In particular, one challenge built into ALFWorld is the need to determine likely locations for common household items (e.g. desklamps will likely be on desks, shelfs, or dressers), making this environment a good fit for LLMs to exploit their pre-trained commonsense knowledge.


HotPotQA \cite{yang2018hotpotqa} with Wikipedia API usage \cite{yao2022react}: (1) search[entity], which returns the first 5 sentences from the corresponding entity wiki page if it exists, or else suggests top-5 similar entities from the Wikipedia search engine, (2) lookup[string], which would return the next sentence in the page containing string, simulating Ctrl+F functionality on the browser. (3) finish[answer], which would finish the current task with answer. 


OpenAGI \cite{openagi} provides an array of datasets, purposefully chosen for benchmark tasks. These datasets employ a carefully curated set of expert models sourced from reputable libraries, such as Hugging Face's transformers and diffusers, as well as GitHub repositories, thereby streamlining the enlargement of their model collection. Furthermore, the selected datasets are meticulously aligned with, or analogous to, the training datasets of the corresponding expert models. Subsequently, an assortment of data augmentation techniques is implemented to refine the initial datasets. This refinement facilitates the creation of intricate, multi-step tasks, explicitly tailored to evaluate the planning and problem-solving abilities of a specific LLM.

API-Bank \cite{li2023api} consists of 53 frequently used API tools, encompassing a variety of applications such as search engines, calendar inquiries, smart home control, hotel bookings, among others. Additionally, it includes 264 annotated dialogues that collectively contain a total of 568 API calls.

APIBench, introduced by Gorilla \cite{patil2023gorilla}, is a large corpus of APIs with complex and often overlapping functionality by scraping ML APIs (models) from public model hubs. For the creation of the dataset, \citet{patil2023gorilla} selected three major model hubs: TorchHub, TensorHub, and HuggingFace. They comprehensively included all API calls from TorchHub, amounting to 94, and from TensorHub, totaling 696. Additionally, they generated 10 synthetic user question prompts for each API using Self-instruct \cite{wang2022self}.

ToolBench \cite{qin2023toolllm} is a dataset designed for instruction-tuning specifically related to tool use and is automatically generated using ChatGPT. As detailed by \citet{qin2023toolllm}, a total of 16,464 real-world RESTful APIs, categorized into 49 distinct groups, were gathered from the RapidAPI Hub. Subsequently, ChatGPT was employed to produce a variety of human instructions incorporating these APIs, which included scenarios involving either a single tool or multiple tools. Lastly, ChatGPT was utilized to identify a feasible solution path, which is a sequence of API calls, for each generated instruction.


ToolAlpaca \cite{tang2023toolalpaca} contains 3938 tool usage instances spanning 426 tools from 50 diverse categories. The instances demonstrate multi-turn interactions between simulated user, assistant, and tool executor agents. On average, each instance has 1-2 function calls and the instructions and responses have lengths of 23 and 36 tokens respectively. 1426 instances involve multiple tool function calls to resolve the request. The tool executor generates realistic JSON responses based on OpenAPI specs.

AgentBench \cite{liu2023agentbench} is a systematically designed multi-dimensional evolving benchmark for evaluating LLMs as agents. For the first time, we include such a wide array of up to 8 real-world challenges to evaluate LLM agents, and establish a unified testing framework and toolkit for agile evaluation. Each challenge is accompanied with real-time interactive environments for testing, in contrast to traditional static-formed NLP datasets. 



MSAgent-Bench, released by \citet{yang2023gpt4tools}, is a comprehensive dataset designed to enable the effective training of an agent. It is comprised of ChatGPT synthetic data and existing instruction-following datasets, totaling 598k dialogues. The dataset is multilingual, containing instances in both Chinese and English, and covers various API categories, including common APIs registered by users or applied through online platforms, and model APIs that can call neural models. It supports multi-turn dialogues, accounting for real-life scenarios where agents may need to request more specific clarifications or receive additional instructions to complete tasks. The dataset also incorporates API-oriented question-answering (QA) tasks, which require agents to offer appropriate suggestions on using various APIs to solve complex tasks, and API-agnostic instructions in both Chinese and English to enhance the agent's ability to follow common instructions and increase user engagement. The data was collected by prompting ChatGPT (gpt-3.5-turbo) to generate instructions, API requests, and answers based on the API calling results.
% BoLLA
% \cite{penedo2023refinedweb}

MineDoJo \cite{fan2022minedojo} offers a set of simulator APIs help researchers develop generally capable, open-ended agents in Minecraft. It builds upon the open-source MineRL codebase.

\begin{table}
\small
\centering
\caption{Caption}
\label{tab:my_label}
\begin{tabularx}{\textwidth}{l|cccccc}
\toprule
Dataset & Language & Instance Type & \# Instances & API type \\
\midrule
OpenAGI & English & Tool Use & 189 & Model API \\
API-Bank  & English & Tool Use & 264 & Common API \\
ToolAlpaca  & English & Tool Use & $3.9 \mathrm{~K}$ & Common API \\
Gorilla & English & Tool Use & $16.4 \mathrm{k}$ & Model API \\
GPT4Tools  & English & Tool Use & $71.4 \mathrm{~K}$ & Model API \\
ToolBench & English & Tool Use & $26.9 \mathrm{~K}$ & Common API \\
MSAgent-Bench & English + Chinese & Tool Use + Common Chat & $598 \mathrm{~K}$ & Common API + Model API \\
\bottomrule
\end{tabularx}
\end{table}


\subsection{Evaluation}
\subsubsection{Subjective Evaluation}

\subsubsection{Objective Evaluation}
ToolEval \cite{qin2023toolllm} is an evaluation framework designed to assess the performance of language learning models (LLMs) in tool usage scenarios. It incorporates two key metrics: Pass Rate and Win Rate. Pass Rate measures the executability of instructions by an LLM, assessing whether instructions are completed successfully within a specified number of actions while excluding false positives. Win Rate, on the other hand, evaluates the quality of the instruction completion by comparing two solution paths for a given instruction, using a set of predefined criteria and the preference of a ChatGPT evaluator. Ultimately, ToolEval provides a comprehensive means of assessing both the completion and the quality of instruction execution by LLMs.

WebShop is evaluated by average score (percentage of desired attributes covered by the chosen product averaged across all episodes) and success rate (percentage of episodes where the chosen product satisfies all requirements) on 500 test instructions.

OpenAGI \cite{openagi}

Current evaluation frameworks for Large Language Models (LLMs) primarily concentrate on single-turn input-output pairs, often neglecting user-provided natural language feedback. Addressing these shortcomings, MINT \cite{wang2023mint} serves as an evaluative benchmark, designed to assess the proficiency of LLMs during multi-turn interactions. It specifically zeroes in on two essential capabilities: (1) tool-augmented task-solving, and (2) capitalizing on natural language feedback. MINT evaluates the tool-augmented task-solving ability of LLMs by scrutinizing the performance enhancement associated with an increasing number of tool-use turns without language feedback. Moreover, it quantifies LLMs' capacity to utilize natural language feedback by measuring the performance improvement when receiving feedback generated by GPT-4.


\subsection{Toolkit and Frameworks}
% \textbf{Closed-source Agents} 



% \noindent\textbf{Open-source Agents} 
Auto-GPT \footnote{https://github.com/Significant-Gravitas/Auto-GPT}, BabyAGI \footnote{https://github.com/yoheinakajima/babyagi}, Langchain \cite{Chase_LangChain_2022}, ModelScope\cite{li2023modelscope}

OpenAgent\cite{xie2023openagents}


Transformers Agent by HuggingFace


\subsection{Open Problems and Future Directions}
\subsubsection{Accuracy and Failure Handling}
Unlike dialogue systems, where the agent and environment take turns, tool-using agents need to additionally decide when to call external tools, which tools to use, and how to use these tools (e.g., reformulating query if results are not helpful), all of which pose additional challenges. Consequently, the supervised finetuning of tool-use agents requires significant human supervision through API call annotations. While prompting-based tool-use requires fewer examples, the specific prompts typically need to be hand-crafted for each tool [Schick et al. 2023]. Moreover, language models are known to be sensitive to the prompt formats in both the zero and few-shot settings [Jiang et al. 2020; Schick and Schütze 2021]. As a result, the communication between language models and external tools typically needs to be cleaned-up by a rule-based parser, which further complicates the prompting setup. Recently, Parisi et al. [2022] and Schick et al. [2023] have made progress on self-supervised learning of tool use with language models, training the language model to only an external tool if this leads to an improved response over the outcome predicted by language model alone. Nevertheless, none of the existing work considers tool use in an interactive setting where an agent can iterate on its behavior according to tool feedback to improve its tool-use ability.

\subsubsection{Scaling Tool Sets}
It is challenging to scale supervised fine-tuning and prompt- ing to a large number of tools with different uses and tools that return large amounts of feedback (e.g., hundreds of search results). One sensible way of tackling this challenge is to treat tools like web browsers as interactive environments, from which experience can be sampled by executing search queries [Nakano et al. 2021; Gur et al. 2022], and optimizing such queries via RL techniques such as policy gradient. Treating tools as interactive environments enables methods that require massive and efficient online simulator access (e.g., Monte Carlo Tree Search for AlphaGo) to be applied to a broader set of real-world problems, such as web navigation and information retrieval. Additionally, situating language models in true knowledge obtained from the environment better grounds the model, avoiding the the Dichotomy of Control problem (e.g., sequence models generating next states without respecting environment transitions) 

% \subsubsection{Failure Handling}





\subsubsection{Personalized Agents}
Machine learning techniques have notably advanced in the realm of classification, a domain wherein, given a set of inputs, a decision must be rendered about a specific output parameter. This encompasses tasks such as identifying objects within an image or deducing the most probable diagnosis based on a patient's symptoms. Nevertheless, the majority of problems deemed to require intelligence extend beyond this straightforward input-output paradigm. Consider the complex ethical dilemma of whether an 87-year-old individual with cardiac complications should undergo chemotherapy to treat bone cancer. While the treatment might extend life expectancy by a year, it could concurrently reduce the quality of life, potentially impeding the individual's capacity to engage with family members. To address such multifaceted issues, any decision-making system must engage directly with the individual, understanding their preferences and core values to derive an optimal decision. The complexity escalates further when accounting for external factors, such as the wishes of a significant other. For instance, if the partner fervently wishes to pursue all available treatment options, while the patient feels content with the life lived, the decision becomes profoundly more intricate.


For instance, \citet{rao2023can} highlighted that ChatGPT has the capability to become more individualized by learning from user engagements and specific preferences. \citet{salemi2023lamp} introduced a benchmark for personalization and proposed the enhancement of large language models (LLMs) by integrating retrieval from user profiles. \citet{wu2022personalized} discussed how pre-trained language models (PLMs) could be personalized using prompts, while \citet{madaan2022memory} suggested incorporating an external memory that includes human feedback for personalizing PLMs. Such personalization can significantly improve user experience by delivering preferred responses, enhancing comprehension of user intentions, and fostering trust and rapport. However, it's crucial to be cognizant of the potential pitfalls. For instance, \citet{deshpande2023toxicity} revealed that giving ChatGPT a specific persona can amplify its toxicity levels by up to sixfold.
Cognitive Architectures \cite{sumers2023cognitive}
